Finding the Transitive Closure of Functional Dependencies using Strategic Port Graph Rewriting

We present a new approach to the logical design of relational databases, based on strategic port graph rewriting. We show how to model relational schemata as attributed port graphs and provide port graph rewriting rules to perform computations on functional dependencies. Using these rules we present a strategic graph program to find the transitive closure of a set of functional dependencies. This program is sound, complete and terminating, assuming that there are no cyclical dependencies in the schema.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{M. Fern\'andez and I. Mackie (Eds.): TERMGRAPH 2018.\\
EPTCS 288, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.288.5}{10.4204/EPTCS.288.5}}
\pdfoutput=1

